Brightest stars of irregular and low-massive spiral galaxies

A search for a correlation between the luminosities of the brightest stars and luminosities of their host galaxies was carried out on archived Hubble Space Telescope (HST) F606W or F555W (V) and F814W (I) images of about 150 nearby galaxies. The sample contains only galaxies with on-going star formation (SF) and with known distances we derived with the TRGB-method. We correlated the average absolute luminosities of the three brightest blue and the three brightest red stars with the luminosity of a host. We found a linear relation for both the blue and the red stars in irregular and low-mass spiral galaxies. Their scatters are sufficiently small (0.m4) to make this relations useful for distance determination for low-mass galaxies. We found that all 31 dwarf galaxies (M_B>-13m) in our sample lack bright stars (M_V(BS)< -7.m0), probably due to the physical conditions that prevent their birth. For galaxies with higher luminosity in the range -18m<M_B<-13m, there is an asymmetry in the distribution of the number of galaxies relative to the linear dependence, indicating an increase in the fraction of galaxies with bright stars.

==> NEWSIMB.TEX <==
%%
%% This is file  `NEWSIMB.TEX',  Strelkov S.A.  30.01.2002
%%
%\newcommand{\vint}{\oint}
%% CyrTUG - LH fonts
% Знак номера
%\newcommand{\No}{\No}
% кавычки типа ,,лапки''
%\newcommand{\glqq}{\qr}
%\newcommand{\grqq}{''}
% кавычки типа <<елочки>>
%\newcommand{\flqq}{<<}
%\newcommand{\frqq}{>>}

%% rtf symbol (rtftoxml.xom coding)

\newcommand{\rtfamp}{\&}           % "&",
\newcommand{\rtflt}{\ifthenelse{\boolean{mmode}}{<}{$<$}} % "<"
\newcommand{\rtfgt}{\ifthenelse{\boolean{mmode}}{>}{$>$}} % ">"
\newcommand{\rtfnbsp}{\~}          % "\~",
\newcommand{\rtfshy}{}             % "\-",
%\newcommand{\rtfshy}{}            % "\_",
\newcommand{\rtfrdquo}{\frqq}      % "rdblquote",
\newcommand{\rtfldquo}{\flqq}      % "ldblquote",
\newcommand{\rtfbull}{\ifthenelse{\boolean{mmode}}{\bullet}{$\bullet$}} % "bullet",
\newcommand{\rtfrsquo}{'}          % "rquote",
\newcommand{\rtflsquo}{`}          % "lquote",
\newcommand{\rtfmdash}{ --- }      % "emdash",
\newcommand{\rtfndash}{ -- }       % "endash",
\newcommand{\rtftab}{}             % "tab",
\newcommand{\rtfline}{}            % "line"
\newcommand{\rtfapos}{'}           % "apos"
\newcommand{\rtf}[1]{\rule{.5em}{em}\verb|rtf{#1}|\rule{.5em}{em}}    % "verbatime"

\newcommand{\rtfgrad}{\ifthenelse{\boolean{mmode}}{^\circ}{$^\circ$}}   % "grad"

\newcommand{\unicode}[1]{\rule{.5em}{em}\verb|unicode{#1}|\rule{.5em}{em}}    % "unicode"
\endinput


==> Newsymbol.tex <==
%%
%% This is file  `NEWSIMB.TEX',  Strelkov S.A.  30.01.2002
%%
%\newcommand{\vint}{\oint}
%% CyrTUG - LH fonts
% Знак номера
%\newcommand{\No}{\No}
% кавычки типа ,,лапки''
%\newcommand{\glqq}{\qr}
%\newcommand{\grqq}{''}
% кавычки типа <<елочки>>
%\newcommand{\flqq}{<<}
%\newcommand{\frqq}{>>}

%% rtf symbol (rtftoxml.xom coding)

\newcommand{\rtfamp}{\&}           % "&",
\newcommand{\rtflt}{\ifthenelse{\boolean{mmode}}{<}{$<$}} % "<"
\newcommand{\rtfgt}{\ifthenelse{\boolean{mmode}}{>}{$>$}} % ">"
\newcommand{\rtfnbsp}{\~}          % "\~",
\newcommand{\rtfshy}{}             % "\-",
%\newcommand{\rtfshy}{}            % "\_",
\newcommand{\rtfrdquo}{\frqq}      % "rdblquote",
\newcommand{\rtfldquo}{\flqq}      % "ldblquote",
\newcommand{\rtfbull}{\ifthenelse{\boolean{mmode}}{\bullet}{$\bullet$}} % "bullet",
\newcommand{\rtfrsquo}{'}          % "rquote",
\newcommand{\rtflsquo}{`}          % "lquote",
\newcommand{\rtfmdash}{ --- }      % "emdash",
\newcommand{\rtfndash}{ -- }       % "endash",
\newcommand{\rtftab}{}             % "tab",
\newcommand{\rtfline}{}            % "line"
\newcommand{\rtfapos}{'}           % "apos"
\newcommand{\rtf}[1]{\rule{.5em}{em}\verb|rtf{#1}|\rule{.5em}{em}}    % "verbatime"

\newcommand{\rtfgrad}{\ifthenelse{\boolean{mmode}}{^\circ}{$^\circ$}}   % "grad"

\newcommand{\unicode}[1]{\rule{.5em}{em}\verb|unicode{#1}|\rule{.5em}{em}}    % "unicode"
%%===================================================
%%===================================================

\def\edtransl#1{\vspace{20pt}\small\bf EDITOR: \
\underline{$\hphantom{\text{Editor's signature}}$}\hfill
\rmfamily Translated by #1}

%\renewcommand{\proofname}{\textbf{Proof}}

\let\rom\textup
\let\emptyset\varnothing
\let\ol\overline
\let\wt\widetilde
\let\wh\widehat
%%\let\<\langle
%%\let\>\rangle
\newcommand{\const}{\operatorname{const}}
%%\renewcommand{\Im}{\operatorname{Im}}
%%\renewcommand{\Re}{\operatorname{Re}}

\makeatletter
\def\m@th{\mathsurround=0pt}
\def\snug{\unskip\kern-\mathsurround}
%%%\newcommand{\mz}{\/\begingroup\everymath{}\m@th$'$\snug\hskip-0.05em\endgroup}
\newcommand{\mz}{'}
\makeatother

\def\href#1#2{{\tt #2}}

\let\q\quad
\let\qq\qquad
\let\br\break
\let\abr\allowbreak
\let\dbr\displaybreak
\let\adbrs\allowdisplaybreaks
\let\nbr\nobreak
\let\nbd\nobreakdash
\let\nmbr\nobreak
\let\lbr\linebreak
\let\pbr\pagebreak
\def\pbrno{\pagebreak\noindent}
\let\hph\hphantom
%
\let\tg\tan
\let\ctg\cot
\let\sc\sec
\let\arctg\arctan
\let\arcctg\arccot
\let\arcsc\arcsec
\let\Arctg\Arctan
\let\Arcctg\Arccot
\let\Arcsc\Arcsec
\let\sh\sinh
\let\ch\cosh
\let\th\tanh
\let\cth\coth
\let\sch\sech
\let\Arsh\asinh
\let\Arch\acosh
\let\Arth\atanh
\let\Arcth\acoth
\let\Arsch\asech
\let\Arcsch\acsch
\let\arsh\asinh
\let\arch\acosh
\let\arth\atanh
\let\arcth\acoth
\let\arsch\asech
\let\arcsch\acsch
%
\endinput


==> PIA_absn.tex <==
%%
%% This is file `PIA_absn.tex',  Strelkov S.A.  30.01.2002
%%
\makeatletter
\def\frontmatter@abstract@produce{%
  \par
  \preprintsty@sw{%
   \do@output@MVL{%
    \vskip\frontmatter@preabstractspace
    \vskip200\p@\@plus1fil
    \penalty-200\relax
    \vskip-200\p@\@plus-1fil
   }%
  }{%
   \addvspace{\frontmatter@preabstractspace}%
  }%
   \begingroup
    \dimen@\baselineskip
    \setbox\z@\vtop{\unvcopy\absbox}%
    \advance\dimen@-\ht\z@\advance\dimen@-\prevdepth
    \@ifdim{\dimen@>\z@}{\vskip\dimen@}{}%
%!
\rule{1pt}{\ht\z@ + \dp\z@}\par
%!!
   \endgroup
   \unvbox\absbox
  \@ifx{\@empty\mini@notes}{}{\mini@notes\par}%
  \addvspace\frontmatter@postabstractspace
}%
\makeatother
\endinput


==> engnames.tex <==
%
% engnames.tex 08.11.2006
%
\makeatletter
\def\contentsname{Contents}
\def\notesname{Notes}
\def\partname{Part}
\def\tocname{Contents}
\def\lofname{List of Figures}
\def\lotname{List of Tables}
\def\refname{REFERENCES}
\def\indexname{Index}
\def\figurename{Fig.}
\def\figuresname{Figures}%
\def\tablename{Table}
\def\tablesname{Tables}%
\def\abstractname{Abstract}
\def\appendixesname{Appendixes}%
\def\appendixname{Appendix}%
\def\acknowledgmentsname{ACKNOWLEDGMENTS}%
\def\fundingname{FUNDING}%
\def\conflictname{CONFLICT OF INTEREST}
\def\journalname{??}
\def\copyrightname{??}
\def\andname{and}
\def\@pacs@name{PACS~numbers~:}%
\def\@ydk@name{УДК~}%
\def\@keywords@name{Key~words:}%
\def\ppname{pp}
\def\numbername{number}
\def\volumename{volume}
\def\Dated@name{dated: }%
\def\Received@name{received }%
\def\Revised@name{revised }%
\def\Accepted@name{accepted }%
\def\Published@name{published }%
\def\Presented@name{}%
%! 08.11.2006
\def\proofname{Proof}
\def\theoremname{Theorem}
\def\lemmaname{Lemma}
\def\propositionname{Proposition}
\def\assertionname{Assertion}
\def\corollaryname{Corollary}
\def\conjecturename{Conjecture}
\def\definitionname{Definition}
\def\remarkname{Remark}
\def\examplename{Conjecture}
%!!
\makeatother
\endinput


==> j_e_add.tex <==
%%
%%  This is file `j_e_add.tex'  Strelkov S.A. 30.01.2002
%%
\pretolerance=500
%\tolerance=1000
% 14.06.2001 Чтобы не было 6 переносов подряд
\tolerance=900
\hyphenpenalty=750
\emergencystretch=5pt
% Львовский стр. 53-54
%\binoppenalty=10000 % Запрещение разрыва после символа бинарной опреации
%\relpenalty=10000   % Запрещение разрыва после символа бинарного отношения
\binoppenalty=700
\relpenalty=500
% Подавляем эффект висячих строк
\clubpenalty=10000 % TeXBook 128,323
\widowpenalty=10000 %
% Включение удвоения символов бинарной операции
% и бинарного отношения при переносе формул
%\input optn % Выключили для английской версии
% Изменение пробелов в математических формулах см. fontmath.ltx
\thinmuskip=3mu
\medmuskip=4mu plus 0mu minus 1mu
\thickmuskip=5mu plus 0mu
%
\frenchspacing
%
\endinput


==> j_r_add.tex <==
%%
%% This is file  j_r_add.tex  Strelkov S.A. 17.06.2002
%%
\hbadness=10000
\vbadness=6000
\hfuzz=2.5pt
\vfuzz=2.5pt
\pretolerance=1500
\tolerance=3000
\hyphenpenalty=2000
\exhyphenpenalty=500
\emergencystretch=5pt
% Львовский стр. 53-54
%\binoppenalty=10000 % Запрещение разрыва после символа бинарной опреации
%\relpenalty=10000   % Запрещение разрыва после символа бинарного отношения
\binoppenalty=700
\relpenalty=500
% Подавляем эффект висячих строк
\clubpenalty=10000 % TeXBook 128,323
\widowpenalty=10000 %
% Включение удвоения символов бинарной операции
% и бинарного отношения при переносе формул
\input optn
% Изменение пробелов в математических формулах см. fontmath.ltx
\thinmuskip=3mu
\medmuskip=4mu plus 0mu minus 1mu
\thickmuskip=5mu plus 0mu
%
\frenchspacing
%
\saythe{\tolerance}
\saythe{\pretolerance}
\saythe{\hyphenpenalty}
\saythe{\exhyphenpenalty}
\saythe{\emergencystretch}
\saythe{\adjdemerits}
\saythe{\doublehyphendemerits}
\saythe{\finalhyphendemerits}
\saythe{\hfuzz}
\saythe{\linepenalty}
\saythe{\looseness}
\saythe{\hbadness}
\saythe{\vbadness}
\saythe{\lefthyphenmin}
\saythe{\righthyphenmin}
\endinput


==> jpack_e.tex <==
%%
%% This is file  `jpack_e.tex',  Strelkov S.A.  31.01.2007
%%
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amsthm}
%\usepackage{oldlfont} %%% Конфликтует с bm.sty
\usepackage{mathtext}
\usepackage[T2A]{fontenc}
\usepackage[cp866]{inputenc}
\usepackage[russian,english]{babel}
\usepackage{literat}
\usepackage{pifont}
\usepackage{bm}
\usepackage{array}
\usepackage{dcolumn}
\usepackage{hhline}
\usepackage{multirow}
\usepackage{graphicx}
\usepackage{rotating}
\usepackage{srcltx_p}
\usepackage{calc}
\usepackage{tabularx}
\usepackage{afterpage}
\usepackage{ifthen}
\usepackage{longtable}
\usepackage{caption2n}
%\usepackage{supertabular}
\RequirePackage{soul}
%\RequirePackage[amsmath]{ntheorem}
\RequirePackage{verbatim}
%
%\theoremseparator{.}
%\theoremindent 0pt
%\theorempreskipamount 6pt plus2pt minus2pt
%\theorempostskipamount 6pt plus2pt minus2pt
%
\RequirePackage{enumerate}
\makeatletter
\setcaptionwidth{\linewidth}
\renewcommand{\captionlabeldelim}{.~}
\renewcommand{\captionlabelfont}{\bfseries}
\renewcommand{\captionfont}{\footnotesize}
\renewcommand \thefigure{\@arabic\c@figure}
\renewcommand \thetable{\@arabic\c@table}
\renewcommand{\arraystretch}{1.5}
\setlength{\extrarowheight}{2pt}
\setlength{\extratabsurround}{2pt}
%%% Как в YADR.CLS
\renewcommand{\topfraction}{.90}
\renewcommand{\dbltopfraction}{.90}
\renewcommand{\bottomfraction}{.90}
\renewcommand{\textfraction}{0.10}
\renewcommand{\floatpagefraction}{0.90}
\renewcommand{\dblfloatpagefraction}{0.90}
\setcounter{topnumber}{4}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{6}
%
\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
\let\PBS=\PreserveBackslash
\def\settabpars#1#2#3{\vskip#1mm \tabcolsep=#2pt \def\arraystretch{#3}}
\newdimen\tabwidth\newdimen\tbwdth
\newcommand{\stretchtab}[2][1.0]{\setbox0=\hbox{\tabcolsep=0sp\ignorespaces#2}
          \setbox1=\hbox{\tabcolsep=1sp\ignorespaces#2}
          \tabwidth=#1\hsize \advance\tabwidth by -\wd0
          %\multiply\tabwidth by 1
          \tbwdth=\wd1\advance\tbwdth by -\wd0
          \divide\tabwidth by \tbwdth
          \tabcolsep=\tabwidth #2}
\newcommand\figcaption{\def\@captype{figure}\caption}
% 26.07.2006 \newcommand\tabcaption{\def\@captype{table}\caption}
\newcommand\tabcaption{\let\captionfont\small\def\@captype{table}\caption}
\renewcommand*\caption@@@normal{%
\parfillskip0pt plus 2fil%
  \caption@label\captiontext\par}
\newcaptionstyle{nonumber}{%
  \usecaptionmargin%
  \captionfont%
  \onelinecaption%
    {{\parbox[t]{\realcaptionwidth}{\parfillskip0pt plus 2fil\captiontext}}}%
    {\parfillskip0pt plus 2fil\captiontext}
}%
\newcommand{\commes}[1]{#1}
%\newcommand{\commes}[1]{\relax}
\def\place@bibnumber@inl#1{#1. }%
\flushbottom
\def\refitem#1{\relax}
%\def\refitem#1{\ifthenelse{\boolean{hmode}}{\protect\newline{}}{}\textbackslash{}refitem\{\hbox{\bfseries{}\itshape{}#1}\}\ifthenelse{\boolean{hmode}}{\protect\linebreak{}}{}}
\makeatother
\endinput


==> jpack_r.tex <==
%%
%% This is file `jpack_r.tex',  Strelkov S.A.  09.02.2007
%%
\usepackage{tipa}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amsthm} % Может использоваться вместо пакета \usepackage[amsmath]{ntheorem}
%\usepackage{oldlfont} %%% Конфликтует с bm.sty
\usepackage{mathtext}
\usepackage[T2A]{fontenc}
\usepackage[cp866]{inputenc}
\usepackage[russian,english]{babel}
\usepackage{literat}
\usepackage{pifont}
\usepackage{bm}
\usepackage{array}
\usepackage{dcolumn}
\usepackage{hhline}
\usepackage{multirow}
\usepackage{graphicx}
\usepackage{rotating}
\usepackage{srcltx_p}
\usepackage{calc}
\usepackage{tabularx}
\usepackage{afterpage}
\usepackage{ifthen}
\usepackage{longtable}
\usepackage{caption2n}
\usepackage{soul}
\usepackage{verbatim}
\usepackage{enumerate}
%\usepackage{tipa}
%
% Может использоваться вместо пакета \usepackage{amsthm}
%
%\usepackage[amsmath]{ntheorem}
%
%\theoremseparator{.}
%\theoremindent 0pt
%\theorempreskipamount 6pt plus2pt minus2pt
%\theorempostskipamount 6pt plus2pt minus2pt
%
\makeatletter
\setcaptionwidth{\linewidth}
\renewcommand{\captionlabeldelim}{.~}
\renewcommand{\captionlabelfont}{\bfseries}
\renewcommand{\captionfont}{\footnotesize}
\renewcommand \thefigure{\@arabic\c@figure}
\renewcommand \thetable{\@arabic\c@table}
\renewcommand{\arraystretch}{1.5}
\setlength{\extrarowheight}{2pt}
\setlength{\extratabsurround}{2pt}
%%% Как в YADR.CLS
\renewcommand{\topfraction}{.90}
\renewcommand{\dbltopfraction}{.90}
\renewcommand{\bottomfraction}{.90}
\renewcommand{\textfraction}{0.10}
\renewcommand{\floatpagefraction}{0.90}
\renewcommand{\dblfloatpagefraction}{0.90}
\setcounter{topnumber}{4}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{6}
%
\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
\let\PBS=\PreserveBackslash
\def\settabpars#1#2#3{\vskip#1mm \tabcolsep=#2pt \def\arraystretch{#3}}
\newdimen\tabwidth\newdimen\tbwdth
\newcommand{\stretchtab}[2][1.0]{\setbox0=\hbox{\tabcolsep=0sp\ignorespaces#2}
          \setbox1=\hbox{\tabcolsep=1sp\ignorespaces#2}
          \tabwidth=#1\hsize \advance\tabwidth by -\wd0
          %\multiply\tabwidth by 1
          \tbwdth=\wd1\advance\tbwdth by -\wd0
          \divide\tabwidth by \tbwdth
          \tabcolsep=\tabwidth #2}
\newcommand\figcaption{\def\@captype{figure}\caption}
% 26.07.2006 \newcommand\tabcaption{\def\@captype{table}\caption}
\newcommand\tabcaption{\let\captionfont\small\def\@captype{table}\caption}
\renewcommand*\caption@@@normal{%
\parfillskip0pt plus 2fil%
  \caption@label\captiontext\par}
\newcaptionstyle{nonumber}{%
  \usecaptionmargin%
  \captionfont%
  \onelinecaption%
    {{\parbox[t]{\realcaptionwidth}{\parfillskip0pt plus 2fil\captiontext}}}%
    {\parfillskip0pt plus 2fil\captiontext}
}%
\newcommand{\commes}[1]{#1}
%\newcommand{\commes}[1]{\relax}
\def\place@bibnumber@inl#1{#1.~}%
\flushbottom
\def\refitem#1{\relax}
%\def\refitem#1{\ifthenelse{\boolean{hmode}}{\protect\newline{}}{}\textbackslash{}refitem\{\hbox{\bfseries{}\itshape{}#1}\}\ifthenelse{\boolean{hmode}}{\protect\linebreak{}}{}}

\makeatother
\endinput


==> maikdoi.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%             This is maikdoi.tex  V 1.1 21.11.2006
%
% Ограничение: можно работать только с ISSN состоящим из цифр;
%              можно задавать \JournalISSNCode(1234-567X)
%              или \JournalCode(X2345671); нет проверки контрольной суммы ISSN.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\ProvidesFile{maikdoi.tex}
              [2006/11/21 v1.1
       add-on for MAIK document class revtex4n]
\typeout{revtex4n Class enhancement: maikdoi.tex for DOI}
%
\makeatletter
%
\def\JournalISSNnumber#1#2#3#4#5#6#7#8#9\@fin{\gdef\@JournalISSNnumber{#1#2#3#4#6#7#8#9}}
\expandafter\JournalISSNnumber\@JournalISSNCode\@fin
\typeout{JournalISSNnumber=\@JournalISSNnumber}
% macros to get and set the basic informations
%\def\journalnumber#1{\xdef\journ@lnumber{\padt@eight@digits{#1}}%
\def\journalnumber#1{\xdef\journ@lnumber{#1}%
%\checksize{journalnumber}8\journ@lnumber{99999999}%
}%
%\let\journ@lnumber=\empty
%
\def\ShortYear#1#2#3#4\@fin{\gdef\@ShortYear{#3#4}}
\expandafter\ShortYear\@TransYearOfIssue\@fin
\typeout{ShortYear=\@ShortYear}
\def\DOIyear#1{\xdef\DOI@year{\padt@two@digits{#1}}\checksize{DOIyear}2\DOI@year{99}}%
%
\def\DOIpsniy#1{\xdef\DOI@psniy{\padt@two@digits{#1}}% psniy - PublicationSerialNumberInYear
\checksize{DOIpsniy}2\DOI@psniy{99}}%
%
\def\DOIartnumber#1{\xdef\DOI@artnumber{\padt@three@digits{#1}}%
\checksize{DOIartnumber}3\DOI@artnumber{999}}
\def\DOI@artnumber{0}
%
\def\doitext#1{\xdef\doit@xtpref{#1}}
%
% a helpful hand of macros
\newif\if@wrongformat \@wrongformatfalse
%
\def\checksize#1#2#3#4{\ifnum#3>#4\PackageError{DOI2module}%
{Numeric value for "#1" to large!\MessageBreak
"#3" specified, but only #2 digits allowed}{Check your input!}
\@wrongformattrue \fi}
%
\newcount\modarg
\newcount\modmod
\newcount\tmp
\def\modulo{\tmp=\modarg\divide\modarg by\modmod\multiply\modarg
by\modmod\multiply\modarg by-1\global\advance\modarg by\tmp}
%
\def\padt@two@digits#1{\ifnum#1<10 0\fi\number#1}%
\def\padt@three@digits#1{\ifnum#1<100 0\fi%
\ifnum#1<10 0\fi\number#1}%
\def\padt@four@digits#1{\ifnum#1<1000 0\fi\ifnum#1<100 0\fi%
\ifnum#1<10 0\fi\number#1}%
\def\padt@five@digits#1{\ifnum#1<10000 0\fi\ifnum#1<1000 0\fi\ifnum#1<100 0\fi%
\ifnum#1<10 0\fi\number#1}%
\def\padt@eight@digits#1{\ifnum#1<1000000 0\fi\ifnum#1<1000000 0\fi\ifnum#1<100000 0%
\fi\ifnum#1<10000 0\fi\ifnum#1<1000 0\fi\ifnum#1<100 0\fi%
\ifnum#1<10 0\fi\number#1}%
%\def\setjahr#1{\xdef\jahr{#1}}
% @pii_digits_weights = (53,47,43,41,37,31,29,23,19,17,13,7,5,3,2);
\def\teilissn#1#2#3#4#5#6#7#8\@fin{%
\if#1X\modarg=10\relax\else\modarg=#1\relax\fi\multiply\modarg by53\advance\tmp by\modarg%
\if#2X\modarg=10\relax\else\modarg=#2\relax\fi\multiply\modarg by47\advance\tmp by\modarg%
\if#3X\modarg=10\relax\else\modarg=#3\relax\fi\multiply\modarg by43\advance\tmp by\modarg%
\if#4X\modarg=10\relax\else\modarg=#4\relax\fi\multiply\modarg by41\advance\tmp by\modarg%
\if#5X\modarg=10\relax\else\modarg=#5\relax\fi\multiply\modarg by37\advance\tmp by\modarg%
\if#6X\modarg=10\relax\else\modarg=#6\relax\fi\multiply\modarg by31\advance\tmp by\modarg%
\if#7X\modarg=10\relax\else\modarg=#7\relax\fi\multiply\modarg by29\advance\tmp by\modarg%
\if#8X\modarg=10\relax\else\modarg=#8\relax\fi\multiply\modarg by23\advance\tmp by\modarg}
\def\teilyear#1#2\@fin{%
\modarg=#1\relax\multiply\modarg by19\advance\tmp by\modarg%
\modarg=#2\relax\multiply\modarg by17\advance\tmp by\modarg}
\def\teilpsniy#1#2\@fin{%
\modarg=#1\relax\multiply\modarg by13\advance\tmp by\modarg%
\modarg=#2\relax\multiply\modarg by7\advance\tmp by\modarg}
\def\teilartnumber#1#2#3\@fin{%
\modarg=#1\relax\multiply\modarg by5\advance\tmp by\modarg%
\modarg=#2\relax\multiply\modarg by3\advance\tmp by\modarg%
\modarg=#3\relax\multiply\modarg by2\advance\tmp by\modarg}
%
% check for all required elements
\def\checkrequirements{
\if!\journ@lnumber!\typein[\answer]{^^JMissing 5-digit
journalnumber for the DOI, please specify:}\journalnumber\answer\fi
%
\ifnum\OF@year=0\typein[\answer]{^^JMissing 4-digit year for the OF
date, please specify:}\OFyear\answer\fi
%
\ifnum\DOI@year=0\typein[\answer]{^^JMissing 4-digit year for the DOI,
please specify:}\DOIyear\answer\fi
{\modarg=\DOI@year\relax\modmod=1000\relax\modulo
\expandafter\setjahr{\padt@three@digits\modarg}}
%
\if!\the\DOI@msnr!\typein[\answer]{^^JMissing 4-digit
manuscript number for the DOI, please specify:}\DOImsnr\answer\fi}
%
% make the package verbose
\def\showDOIargs{%
\typeout{^^JList of arguments for this DOI2 generation
^^J==========================================
^^JDOI-prefix :\space\maikpraefix
^^JISSN number:\space\journ@lnumber
^^JDOI-year\space\space\space:\space\DOI@year
^^JIn-Year-No.:\space\DOI@psniy
^^JArticle-No.:\space\DOI@artnumber
^^J==========================================}}
%
% perform the calculation
\def\DOIt{\if@wrongformat
   \typeout{Wrong format of at least one required value,^^Jno
            DOI could be generated.^^J}%
\else
   \edef\doit@xtcode{%
   \maikpraefix\journ@lnumber\DOI@year\DOI@psniy\DOI@artnumber}%
   \tmp=0\relax%
   \expandafter\teilissn\journ@lnumber\@fin%
   \expandafter\teilyear\DOI@year\@fin%
   \expandafter\teilpsniy\DOI@psniy\@fin%
   \expandafter\teilartnumber\DOI@artnumber\@fin%
   \modarg=\tmp\modmod=11\relax\modulo
   \ifnum\modarg<10\edef\checksum{\the\modarg}\else\edef\checksum{X}%
   \fi
   \edef\doit@xtcode{\doit@xtcode\checksum}
   \edef\doit@xt{\doit@xtpref\doit@xtcode}
   \showDOIargs
   \typeout{Calculated DOI:\space\space\doit@xtcode
   ^^J^^JVerbose:^^J\doit@xt^^J}
\fi
}
%
% set the defaults - the basics at least
%\def\springerpraefix{10.1007/s}
%!\def\maikpraefix{10.1134/S}
\doitext{\relax}%
%
\journalnumber{\@JournalISSNnumber}
\typeout{journalnumber=\journ@lnumber}
\DOIyear{\@ShortYear}
\typeout{DOIyear=\DOI@year}
\DOIpsniy{\@PublicationSerialNumberInYear}
\typeout{DOIpsniy=\DOI@psniy}
\makeatother
\endinput
%% End of file `maik.doi'


==> maikthm.tex <==
%\theoremstyle{plain}
%\newtheorem{theorem}{Теорема} %
%\newtheorem{lemmma}{Лемма}
%\newtheorem{proposition}{Предложение}
%\theoremstyle{definition}
%\newtheorem{axiom}{Аксиома}
%\newtheorem{corollary}{Следствие}
%\newtheorem{example}{Пример}
%\theoremstyle{remark}
%\newtheorem{remark}{Замечание}
%\newtheorem{case}{Случай}
%
\advance \topsep by 2pt
\newdimen\remarktopsep
\remarktopsep=\topsep
\divide\remarktopsep by 2
%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section] %
\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{problem}{Problem}
\newtheorem{hypothesis}{Hypothesis}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{example}{Example}[section]
\theoremstyle{remark}
\newtheorem{remark}{Remark}[section]
%\newtheorem{case}{Case}[section]
%\renewcommand{\thedefinition}{\Alph{definition}} - если нужна буквенная нумерация
%
\newtheoremstyle{aplain}% name
{\topsep}%      Space above
{\topsep}%      Space below
{\itshape}%         Body font
{}%         Indent amount (empty = no indent, \parindent = para indent)
{\bfseries}% Thm head font
{.}%        Punctuation after thm head
{ }%     Space after thm head: " " = normal interword space; \newline = linebreak
{#1~#3}%         Thm head spec (can be left empty, meaning `normal')
\newtheoremstyle{adefinition}% name
{\topsep}%      Space above
{\topsep}%      Space below
{}%         Body font
{}%         Indent amount (empty = no indent, \parindent = para indent)
{\bfseries}% Thm head font
{.}%        Punctuation after thm head
{ }%     Space after thm head: " " = normal interword space; \newline = linebreak
{#1~#3}%         Thm head spec (can be left empty, meaning `normal')
\newtheoremstyle{aremark}% name
{\remarktopsep}%      Space above
{\remarktopsep}%      Space below
{}%         Body font
{}%         Indent amount (empty = no indent, \parindent = para indent)
{\bfseries}% Thm head font
{.}%        Punctuation after thm head
{ }%     Space after thm head: " " = normal interword space; \newline = linebreak
{#1~#3}%         Thm head spec (can be left empty, meaning `normal')
\theoremstyle{aplain}
\newtheorem{atheorem}{Theorem} %
\newtheorem{alemma}{Lemma}
\newtheorem{aproposition}{Proposition}
\newtheorem{acorollary}{Corollary}
\newtheorem{aproblem}{Problem}
%\newtheorem{ahypothesis}{Hypothesis}
\newtheorem{ahypothesis}{Conjecture}
\theoremstyle{adefinition}
\newtheorem{adefinition}{Definition}
\newtheorem{aexample}{Example}
\newtheorem{aproperties}{Properties}
\theoremstyle{aremark}
\newtheorem{aremark}{Remark}
\newtheorem{acase}{Case}


==> newsimb.tex <==
%%
%% This is file  `NEWSIMB.TEX',  Strelkov S.A.  30.01.2002
%%
%\newcommand{\vint}{\oint}
%% CyrTUG - LH fonts
% Знак номера
%\newcommand{\No}{\No}
% кавычки типа ,,лапки''
%\newcommand{\glqq}{\qr}
%\newcommand{\grqq}{''}
% кавычки типа <<елочки>>
%\newcommand{\flqq}{<<}
%\newcommand{\frqq}{>>}

%% rtf symbol (rtftoxml.xom coding)

\newcommand{\rtfamp}{\&}           % "&",
\newcommand{\rtflt}{\ifthenelse{\boolean{mmode}}{<}{$<$}} % "<"
\newcommand{\rtfgt}{\ifthenelse{\boolean{mmode}}{>}{$>$}} % ">"
\newcommand{\rtfnbsp}{\~}          % "\~",
\newcommand{\rtfshy}{}             % "\-",
%\newcommand{\rtfshy}{}            % "\_",
\newcommand{\rtfrdquo}{\frqq}      % "rdblquote",
\newcommand{\rtfldquo}{\flqq}      % "ldblquote",
\newcommand{\rtfbull}{\ifthenelse{\boolean{mmode}}{\bullet}{$\bullet$}} % "bullet",
\newcommand{\rtfrsquo}{'}          % "rquote",
\newcommand{\rtflsquo}{`}          % "lquote",
\newcommand{\rtfmdash}{ --- }      % "emdash",
\newcommand{\rtfndash}{ -- }       % "endash",
\newcommand{\rtftab}{}             % "tab",
\newcommand{\rtfline}{}            % "line"
\newcommand{\rtfapos}{'}           % "apos"
\newcommand{\rtf}[1]{\rule{.5em}{em}\verb|rtf{#1}|\rule{.5em}{em}}    % "verbatime"

\newcommand{\rtfgrad}{\ifthenelse{\boolean{mmode}}{^\circ}{$^\circ$}}   % "grad"

\newcommand{\unicode}[1]{\rule{.5em}{em}\verb|unicode{#1}|\rule{.5em}{em}}    % "unicode"
\endinput


==> optn.tex <==
%%
%% This is file `optn.tex',  Strelkov S.A.  30.01.2002
%%
\begingroup
\catcode`\+\active\gdef+{\mathchar8235\nobreak\discretionary{}{\usefont{OT1}{cmr}{m}{n}\char43}{}}
\catcode`\-\active\gdef-{\mathchar8704\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char0}{}}
\catcode`\=\active\gdef={\mathchar12349\nobreak\discretionary{}{\usefont{OT1}{cmr}{m}{n}\char61}{}}
\endgroup
\def\cdot{\mathchar8705\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char1}{}}
\def\times{\mathchar8706\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char2}{}}
\mathcode`\==32768
\mathcode`\+=32768
\mathcode`\-=32768
% Класс математического символа TeXBook стрю 185-186
% 2 --- Бинарный оператор
% 3 --- Отношение
% <\equiv =\mathchar"3211>
\def \equiv   {\mathchar8721\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char17}{}}% "2211
% A.2.2~Бинарные отношения~LaTeX'a
% <\subseteq =\mathchar"3212>
\def \subseteq{\mathchar8722\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char18}{}} % "2222
% <\supseteq =\mathchar"3213>
\def \supseteq{\mathchar8723\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char19}{}}
\def \leq     {\mathchar8724\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char20}{}}
\def \geq     {\mathchar8725\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char21}{}}
\def \sim     {\mathchar8728\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char24}{}}
\def \approx  {\mathchar8729\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char25}{}}
\def \subset  {\mathchar8730\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char26}{}}
\def \supset  {\mathchar8731\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char27}{}}
\def \ll      {\mathchar8732\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char28}{}}
\def \gg      {\mathchar8733\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char29}{}}
\def \pm      {\mathchar8710\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char6}{}}
\def \mp      {\mathchar8711\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char7}{}}
\def \in      {\mathchar8754\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char50}{}}
\def \ni      {\mathchar8755\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char51}{}}
% См. TeXBook стр. 510-511
% Некоторые символы имеют альтернативные имена, которые так широко используются,
% что plain TeX имеет для них по две или более командные последовательности:
% \ne или \neq (то же, что \not=)
% \le          (то же, что \leq)
% \ge          (то же, что \geq)
% (то же, что )
% (то же, что )
% (то же, что )
%<\prec =\mathchar"321E>
\def \prec    {\mathchar"321E\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"1E}{}}
%<\succ =\mathchar"321F>
\def \succ    {\mathchar"321F\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"1F}{}}
%<\preceq =\mathchar"3216>
\def \preceq  {\mathchar"3216\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"16}{}}
%<\succeq =\mathchar"3217>
\def \succeq  {\mathchar"3217\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"17}{}}
%<\simeq =\mathchar"3227>
\def \simeq  {\mathchar"3227\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"27}{}}
%<\cong =macro:->\mathrel {\mathpalette \@vereq \sim }>
%<\doteq =\long macro:->\DOTSB \mathrel {\mathop {\kern 0pt =}\limits ^{\textstyle .}}>
%<\sqsubseteq =\mathchar"3276>
\def \sqsubseteq {\mathchar"3276\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"76}{}}
%<\sqsupseteq =\mathchar"3277>
\def \sqsupseteq {\mathchar"3277\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"77}{}}
%<\smile =\mathchar"315E>
\def \smile   {\mathchar"315E\nobreak\discretionary{}{\usefont{OML}{cmm}{m}{n}\char"5E}{}}
%<\frown =\mathchar"315F>
\def \frown   {\mathchar"315F\nobreak\discretionary{}{\usefont{OML}{cmm}{m}{n}\char"5F}{}}
%<\perp =\mathchar"323F>
\def \perp    {\mathchar"323F\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"3F}{}}
%<\models =macro:->\mathrel {|}\joinrel \Relbar >
%<\mid =\mathchar"326A>
\def \mid     {\mathchar"326A\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"6A}{}}
%<\parallel =\mathchar"326B>
\def \parallel {\mathchar"326B\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"6B}{}}
%<\vdash =\mathchar"3260>
\def \vdash  {\mathchar"3260\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"60}{}}
%<\dashv =\mathchar"3261>
\def \dashv  {\mathchar"3261\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"61}{}}
%<\propto =\mathchar"322F>
\def \propto  {\mathchar"322F\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"2F}{}}
%<\asymp =\mathchar"3210>
\def \asymp  {\mathchar"3210\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"10}{}}
% latexsym
%<\sqsubset =\mathchar"3440>
\def \sqsubset {\mathchar"3440\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"40}{}}
%<\sqsupset =\mathchar"3441>
\def \sqsupset {\mathchar"3441\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"41}{}}
% A.2.2~Бинарные отношения~AMS
%<\leqslant =\mathchar"3436>
\def \leqslant {\mathchar"3436\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"36}{}}
%<\geqslant =\mathchar"343E>
\def \geqslant {\mathchar"343E\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"3E}{}}
%<\eqslantless =\mathchar"3430>
\def \eqslantless {\mathchar"3430\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"30}{}}
%<\eqslantgtr =\mathchar"3431>
\def \eqslantgtr {\mathchar"3431\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"31}{}}
%<\lesssim =\mathchar"342E>
%\def \lessim {\mathchar"342E\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"2E}{}}
%<\gtrsim =\mathchar"3426>
\def \gtrsim {\mathchar"3426\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"26}{}}
%<\lll =\mathchar"346E>
\def \lll {\mathchar"346E\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"6E}{}}
%<\ggg =\mathchar"346F>
\def \ggg {\mathchar"346F\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"6F}{}}
%<\lessgtr =\mathchar"3437>
\def \lessgtr {\mathchar"3437\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"37}{}}
%<\gtrless =\mathchar"343F>
\def \gtrless {\mathchar"343F\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"3F}{}}
%<\doteqdot =\mathchar"342B>
\def \doteqdot {\mathchar"342B\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"2B}{}}
%<\eqcirc =\mathchar"3450>
\def \eqcirc {\mathchar"3450\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"50}{}}
%<\circeq =\mathchar"3424>
\def \circeq {\mathchar"3424\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"24}{}}
%<\triangleq =\mathchar"342C>
\def \triangleq {\mathchar"342C\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"2C}{}}
%<\risingdotseq =\mathchar"343A>
\def \risingdotseq {\mathchar"343A\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"3A}{}}
%<\fallingdotseq =\mathchar"343B>
\def \fallingdotseq {\mathchar"343B\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"3B}{}}
%<\subseteqq =\mathchar"346A>
\def \subseteqq {\mathchar"346A\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"6A}{}}
%<\supseteqq =\mathchar"346B>
\def \supseteqq {\mathchar"346B\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"6B}{}}
%<\vartriangleleft =\mathchar"3443>
\def \vartriangleleft {\mathchar"3443\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"43}{}}
%<\vartriangleright =\mathchar"3442>
\def \vartriangleright {\mathchar"3442\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"42}{}}
% A.2.3~Бинарные отношения~AMS~с~отрицанием
\def \neq      {\hbox{\text{\kern0.3em{\usefont{OMS}{cmsy}{m}{n}\char54}=}\kern0.3em}\nobreak\discretionary{}{{\usefont{OMS}{cmsy}{m}{n}\char54}=\kern0.3em}{}}
\let\ne=\neq
% <\nless =\mathchar"3504>
\def \nless   {\mathchar"3504\nobreak\discretionary{}{{\usefont{U}{msb}{m}{n}\char"04}}{}}
%<\in =\mathchar"3232>
%<\notin =macro:->\mathrel {\m@th \mathpalette \c@ncel \in }>
%<\nparallel =\mathchar"352C>
\def \nparallel {\mathchar"352C\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"2C}{}}
%<\nsubseteq =\mathchar"352A>
\def \nsubseteq {\mathchar"352A\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"2A}{}}
%<\nsupseteq =\mathchar"352B>
\def \nsupseteq {\mathchar"352B\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"2B}{}}
% A.3~Бинарные~операции
%<\circ =\mathchar"220E>
\def \circ {\mathchar"220E\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"0E}{}}
%<\bigcirc =\mathchar"220D>
\def \bigcirc {\mathchar"220D\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"0D}{}}
%<\div =\mathchar"2204>
\def \div {\mathchar"2204\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"04}{}}
%<\diamond =\mathchar"2205>
\def \diamond {\mathchar"2205\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"05}{}}
%<\ast =\mathchar"2203>
\def \ast {\mathchar"2203\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"03}{}}
%<\star =\mathchar"213F>
\def \star {\mathchar"213F\nobreak\discretionary{}{\usefont{OML}{cmm}{m}{n}\char"3F}{}}
%<\cap =\mathchar"225C>
\def \cap {\mathchar"225C\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"5C}{}}
%<\cup =\mathchar"225B>
\def \cup {\mathchar"225B\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"5B}{}}
%<\sqcap =\mathchar"2275>
\def \sqcap {\mathchar"2275\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"75}{}}
%<\sqcup =\mathchar"2274>
\def \sqcup {\mathchar"2274\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"74}{}}
%<\wedge =\mathchar"225E>
\def \wedge {\mathchar"225E\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"5E}{}}
%<\vee =\mathchar"225F>
\def \vee {\mathchar"225F\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"5F}{}}
%<\oplus =\mathchar"2208>
\def \oplus {\mathchar"2208\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"08}{}}
%<\ominus =\mathchar"2209>
\def \ominus {\mathchar"2209\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"09}{}}
%<\otimes =\mathchar"220A>
\def \otimes {\mathchar"220A\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"0A}{}}
%<\odot =\mathchar"220C>
\def \odot {\mathchar"220C\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"0C}{}}
%<\Cap =\mathchar"2465>
\def \Cap {\mathchar"2465\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"65}{}}
%<\Cup =\mathchar"2464>
\def \Cup {\mathchar"2464\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"64}{}}
% A.4~Стрелки
%<\leftarrow =\mathchar"3220>
\def \leftarrow  {\mathchar"3220\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"20}{}}
%<\rightarrow =\mathchar"3221>
\def \rightarrow  {\mathchar"3221\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"21}{}}
%<\to =\mathchar"3221>
\def \to  {\mathchar"3221\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"21}{}}
%<\longleftarrow =\long macro:->\DOTSB \leftarrow \protect \joinrel \protect \relbar >
%<\longrightarrow =\long macro:->\DOTSB \protect \relbar \protect \joinrel \rightarrow >
%<\Leftarrow =\mathchar"3228>
\def \Leftarrow  {\mathchar"3228\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"28}{}}
%<\Rightarrow =\mathchar"3229>
\def \Rightarrow  {\mathchar"3229\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"29}{}}
%<\Longleftarrow =\long macro:->\DOTSB \Leftarrow \protect \joinrel \protect \Relbar >
%<\Longrightarrow =\long macro:->\DOTSB \protect \Relbar \protect \joinrel \Rightarrow >
%<\leftrightarrow =\mathchar"3224>
\def \leftrightarrow  {\mathchar"3224\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"24}{}}
%<\longleftrightarrow =\long macro:->\DOTSB \leftarrow \joinrel \rightarrow >
%<\Leftrightarrow =\mathchar"322C>
\def \Leftrightarrow  {\mathchar"322C\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"2C}{}}
%<\Longleftrightarrow =\long macro:->\DOTSB \Leftarrow \joinrel \Rightarrow >
%<\uparrow =macro:->\delimiter "3222378 >
%<\downarrow =macro:->\delimiter "3223379 >
%<\Uparrow =macro:->\delimiter "322A37E >
%<\Downarrow =macro:->\delimiter "322B37F >
%<\updownarrow =macro:->\delimiter "326C33F >
%<\Updownarrow =macro:->\delimiter "326D377 >
%<\leftleftarrows =\mathchar"3412>
\def \leftleftarrows {\mathchar"3412\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"12}{}}
%<\rightrightarrows =\mathchar"3413>
\def \rightrightarrows {\mathchar"3413\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"13}{}}
%<\leftrightarrows =\mathchar"341C>
\def \leftrightarrows {\mathchar"341C\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"1C}{}}
%<\rightleftarrows =\mathchar"341D>
\def \rightleftarrows {\mathchar"341D\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"1D}{}}
%<\upuparrows =\mathchar"3414>
\def \upuparrows {\mathchar"3414\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"14}{}}
%<\downdownarrows =\mathchar"3415>
\def \downdownarrows {\mathchar"3415\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"15}{}}
%<\nLeftarrow =\mathchar"353A>
\def \nLeftarrow {\mathchar"353A\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"3A}{}}
%<\nRightarrow =\mathchar"353B>
\def \nRightarrow {\mathchar"353B\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"3B}{}}
\endinput
%\DeclareFontEncoding{OML}{}{}
%\DeclareFontEncoding{OMS}{}{}
%\DeclareFontEncoding{OMX}{}{}
%\DeclareFontEncoding{U}{}{\noaccents@}
%\DeclareFontSubstitution{OML}{cmm}{m}{it}
%\DeclareFontSubstitution{OMS}{cmsy}{m}{n}
%\DeclareFontSubstitution{OMX}{cmex}{m}{n}
%\DeclareFontSubstitution{U}{cmr}{m}{n}


==> rusnames.tex <==
%%
%% This is file `rusnames.tex',  Strelkov S.A.  08.11.2006
%%
\makeatletter
\def\contentsname{СОДЕРЖАНИЕ}
\def\notesname{Примечания}
\def\partname{Часть}
\def\tocname{Содержание}
\def\lofname{Cписок илл.}
\def\lotname{Cписок табл.}
\def\refname{СПИСОК ЛИТЕРАТУРЫ}
\def\indexname{Указатель}
\def\figurename{Рис.}
\def\figuresname{Рис.}%
\def\tablename{Таблица}
\def\tablesname{Таблицы}%
\def\abstractname{}
\def\appendixesname{ПРИЛОЖЕНИЯ}%
\def\appendixname{ПРИЛОЖЕНИЕ}%
\def\acknowledgmentsname{БЛАГОДАРНОСТИ}
\def\journalname{??}
\def\copyrightname{??}
\def\andname{\relax}
\def\@pacs@name{PACS~numbers~:}%
\def\@ydk@name{УДК~}%
%\def\@keywords@name{Key~words:}%
\def\@keywords@name{Ключевые~слова:}%
\def\ppname{pp}
\def\numbername{number}
\def\volumename{volume}
\def\Dated@name{dated: }%
\def\Received@name{Поступила в редакцию }%
\def\Revised@name{после доработки }%
\def\Accepted@name{принята к публикации }%
\def\Published@name{published }%
\def\Presented@name{}%
% 08.11.2006
\def\proofname{{\cyr\CYRD~\cyro~\cyrk~\cyra~\cyrz~\cyra~\cyrt~\cyre~\cyrl~\cyrsftsn~\cyrs~\cyrt~\cyrv~\cyro}}%
\def\theoremname{{\cyr\CYRT~\cyre~\cyro~\cyrr~\cyre~\cyrm~\cyra}}
\def\lemmaname{{\cyr\CYRL~\cyre~\cyrm~\cyrm~\cyra}}
\def\propositionname{{\cyr\CYRS~\cyru~\cyrzh~\cyrd~\cyre~\cyrn~\cyri~\cyre}}
\def\assertionname{{\cyr\CYRU~\cyrt~\cyrv~\cyre~\cyrr~\cyrzh~\cyrd~\cyre~\cyrn~\cyri~\cyre}}
\def\corollaryname{{\cyr\CYRZ~\cyra~\cyrk~\cyrl~\cyryu~\cyrch~\cyre~\cyrn~\cyri~\cyre}}
\def\conjecturename{{\cyr\CYRP~\cyrr~\cyre~\cyrd~\cyrp~\cyro~\cyrl~\cyro~\cyrzh~\cyre~\cyrn~\cyri~\cyre}}
\def\definitionname{{\cyr\CYRO~\cyrp~\cyrr~\cyre~\cyrd~\cyrl~\cyre~\cyrn~\cyri~\cyre}}
\def\remarkname{{\cyr\CYRZ~\cyra~\cyrm~\cyre~\cyrch~\cyra~\cyrn~\cyri~\cyre}}
\def\examplename{{\cyr\CYRP~\cyrr~\cyri~\cyrm~\cyre~\cyrr}}
\makeatother
\endinput


==> sao_cmd.tex <==
% САО РАН
\def\saoname{Special Astrophysical Observatory,  Russian Academy of Sciences,
Nizhnii Arkhyz, 369167 Russia}
\def\saonamer{Специальная астрофизическая обсерватория РАН, Нижний Архыз, 369167
Россия}
% КрАО
\def\craoname{Crimean Astrophysical Observatory, Russian Academy of Sciences,
Nauchny, 298409 Russia}
\def\craonamer{Крымская астрофизическая обсерватория РАН, Научный, 298409
Россия}
% Крымский университет
\def\crunivname{V.~I.~Vernadsky Crimean Federal University, Simferopol, 295007 Russia}
\def\crunivnamer{Крымский федеральный университет им.~В.~И.~Вернадского, Симферополь, 295007
Россия}
% ИКИ
\def\ikiname{Space Research Institute, Russian Academy of Sciences, Moscow, 117997 Russia}
\def\ikinamer{Институт космических исследований РАН, Москва, 117997 Россия}
% АКЦ ФИАН
\def\aktsname{Astro Space Center, Lebedev Physical Institute, Russian Academy of Sciences,
Moscow, 117997 Russia}
\def\aktsnamer{Астрокосмический центр Физического института им. П.~Н.~Лебедева РАН, Москва, 117997
Россия}
% ИТМО
\def\itmoname{National Research University of Information Technologies, Mechanics and Optics,
St.~Petersburg, 197101 Russia}
\def\itmonamer{Национальный исследовательский университет информационных технологий,
механики и оптики, Санкт-Петербург, 197101 Россия}
% ИПА
\def\ipaname{Institute of Applied Astronomy,  Russian Academy of Sciences,
St.~Petersburg, 191187 Russia}
\def\ipanamer{Институт прикладной астрономии РАН, Санкт-Петербург, 191187 Россия}
% ШАО
\def\shaoname{Shamakhy Astrophysical Observatory named after Nasreddin Tusi,
Azerbaijan National Academy of Sciences, Shamakhy, AZ 5626
Azerbaijan}
\def\shaonamer{Шемахинская астрофизическая обсерватория им.~Насреддина~Туси АНАН, Шамахы, AZ 5626
Азербайджан}
% КФУ
\def\kfuname{Kazan (Volga Region) Federal University, Kazan, 420008 Russia}
\def\kfunamer{Казанский (Приволжский) федеральный университет, Казань, 420008 Россия}
% ГАИШ
\def\gaishname{Sternberg Astronomical Institute, Moscow State University, Moscow, 119234 Russia}
\def\gaishnamer{Государственный астрономический институт им.~П.~К.~Штернберга
Московского государственного университета им.~М.~В.~Ломоносова,
Москва, 119234 Россия}
% МГУ
\def\mguname{Moscow State University, Moscow, 119234 Russia}
\def\mgunamer{Московский государственный университет им.~М.~В.~Ломоносова,
Москва, 119234 Россия}
% ЮФУ
\def\yufuname{Southern Federal University, Rostov-on-Don, 344006 Russia}
\def\yufunamer{Южный федеральный университет, Ростов-на-Дону, 344006 Россия}
% УрФУ
\def\urfuname{Ural Federal University named after the First President of Russia
B.~N.~Yeltsin, Yekaterinburg, 620000 Russia}
\def\urfunamer{Уральский федеральный университет им.~Первого президента России
Б.~Н.~Ельцина, Екатеринбург, 620000 Россия}
% Коуровка
\def\kourname{Kourovka Astronomical Observatory named after K.~A.~Barkhatova,
Ural Federal University named after the First President of Russia
B.~N.~Yeltsin, Yekaterinburg, 620000 Russia}
\def\kournamer{Коуровская астрономическая обсерватория им.~К.~А.~Бархатовой
Уральского федерального университета им.~Первого президента России
Б.~Н.~Ельцина, Екатеринбург, 620000 Россия}
% ГАО СПб
\def\pgaoname{Central (Pulkovo) Astronomical Observatory,  Russian Academy of Sciences,
St.~Petersburg, 196140 Russia}
\def\pgaonamer{Главная (Пулковская) астрономическая обсерватория РАН, Санкт-Петербург, 196140
Россия}
% ГАО Киев
\def\kgaoname{Main Astronomical Observatory, National Academy of Sciences of Ukraine,
Kyiv, 03143 Ukraine}
\def\kgaonamer{Главная астрономическая обсерватория НАНУ, Киев, 03143 Украина}
% СПбГУ
\def\spbguname{St.~Petersburg University, St.~Petersburg, 199034 Russia}
\def\spbgunamer{Санкт-Петербургский государственный университет, Санкт-Петербург, 199034
Россия}
% Калмыцкий университет Элиста
\def\kalmguname{Kalmyk State University named after B.~B.~Gorodovikov, Elista, 358000 Russia}
\def\kalmgunamer{Калмыцкий государственный университет им.~Б.~Б.~Городовикова, Элиста, 358000
Россия}
% Университет Киев
\def\kievuname{Taras Shevchenko National University of Kyiv, Kyiv, 01601 Ukraine}
\def\kievunamer{Киевский национальный университет им.~Тараса Шевченко, Киев, 01601
Украина}
% ИНАСАН
\def\inasanname{Institute of Astronomy,  Russian Academy of Sciences, Moscow, 119017 Russia}
\def\inasannamer{Институт астрономии РАН, Москва, 119017 Россия}


%******* SPECIAL SIGNS AND CHARACTERS FOR MATH MODE *******
%
\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}

\def\sq{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\squareforqed
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}

\def\sun{\hbox{$\odot$}}

\def\la{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\sim\cr}}}}}

\def\ga{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\sim\cr}}}}}

\def\degr{\hbox{$^\circ$}}

\def\arcmin{\hbox{$^\prime$}}

\def\arcsec{\hbox{$^{\prime\prime}$}}

\def\utw{\smash{\rlap{\lower5pt\hbox{$\sim$}}}}

\def\udtw{\smash{\rlap{\lower6pt\hbox{$\approx$}}}}

\def\fa{\hbox{$\,.\!\!^{\rm a}$}}

\def\fd{\hbox{$\,.\!\!^{\rm d}$}}

\def\fh{\hbox{$\,.\!\!^{\rm h}$}}

\def\fm{\hbox{$\,.\!\!^{\rm m}$}}

\def\fs{\hbox{$\,.\!\!^{\rm s}$}}

\def\fdg{\hbox{$\,.\!\!^\circ$}}

\def\farcm{\hbox{$\,.\mkern-4mu^\prime$}}

\def\farcs{\hbox{$\,.\!\!^{\prime\prime}$}}

\def\fp{\hbox{$\,.\!\!^{\scriptscriptstyle\rm p}$}}

\def\cor{\mathrel{\mathchoice {\hbox{$\widehat=$}}{\hbox{$\widehat=$}}
{\hbox{$\scriptstyle\hat=$}}
{\hbox{$\scriptscriptstyle\hat=$}}}}

\def\sol{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr\sim\cr<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr\sim\cr
<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr\sim\cr
<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
\sim\cr<\cr}}}}}

\def\sog{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr\sim\cr>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr\sim\cr
>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
\sim\cr>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
\sim\cr>\cr}}}}}

\def\lse{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\simeq\cr}}}}}

\def\gse{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\simeq\cr}}}}}

\def\grole{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\noalign{\vskip-1.5pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\noalign{\vskip-1.5pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\noalign{\vskip-1pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\noalign{\vskip-0.5pt}<\cr}}}}}

\def\leogr{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\noalign{\vskip-1.5pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\noalign{\vskip-1.5pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\noalign{\vskip-1pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\noalign{\vskip-0.5pt}>\cr}}}}}

\def\loa{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\approx\cr}}}}}

\def\goa{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\approx\cr}}}}}

\def\diameter{{\ifmmode\mathchoice
{\ooalign{\hfil\hbox{$\displaystyle/$}\hfil\crcr
{\hbox{$\displaystyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\textstyle/$}\hfil\crcr
{\hbox{$\textstyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\scriptstyle/$}\hfil\crcr
{\hbox{$\scriptstyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\scriptscriptstyle/$}\hfil\crcr
{\hbox{$\scriptscriptstyle\mathchar"20D$}}}}
\else{\ooalign{\hfil/\hfil\crcr\mathhexbox20D}}%
\fi}}

\def\getsto{\mathrel{\mathchoice {\vcenter{\offinterlineskip
\halign{\hfil
$\displaystyle##$\hfil\cr\gets\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr\gets
\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr\gets
\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
\gets\cr\to\cr}}}}}

\def\lid{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr<\cr
\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr<\cr
\noalign{\vskip1pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr
\noalign{\vskip0.9pt}=\cr}}}}}

\def\gid{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr>\cr
\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr>\cr
\noalign{\vskip1pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr
\noalign{\vskip0.9pt}=\cr}}}}}

%********** ABBREVIATIONS OF THE OFT-REFERENCED JOURNALS ***********

% *** Астрофизические исследования % русск. версия журнала САО до 1993 г.
\newcommand{\air}{Астрофиз. исслед. (Известия Спец. астрофиз. обс.) }
% *** Астрофизические исследования % англ. версия журнала САО до 1993 г.
\newcommand{\aireng}{Astrofiz. Issled.: Izvestiya Spets. Astrofiz. Obs. }
% *** Astrophysical Bulletin % англ. версия журнала САО с 2007 г.
\newcommand{\ab}{Astrophysical Bulletin }
% *** Астрофизический бюллетень % русск. версия журнала САО с 2007 г.
\newcommand{\abr}{Астрофизический бюллетень }
% *** Astronomy and Astrophysics
\newcommand{\aaa}{Astron. and Astrophys. }
\newcommand{\aap}{Astron. and Astrophys. }
% *** Astronomy and Astrophys. Supplement Series
\newcommand{\aas}{Astron. and Astrophys. Suppl. }
\newcommand{\aaps}{Astron. and Astrophys. Suppl. }
% *** Astronomy and Astrophysics Review
\newcommand{\aar}{Astron. Astrophys. Rev. }
% *** Astronomical Journal
\newcommand{\aj}{Astron.~J. }
% *** Astrophysical Journal
\newcommand{\apj}{Astrophys.~J. }
% *** Astrophysical Journal Supplement Series
\newcommand{\apjs}{Astrophys.~J. Suppl. }
% *** Astrophysics and Space Science
\newcommand{\apss}{Astrophys. and Space Sci. }
% *** Annual Review of Astronomy and Astrophys.
\newcommand{\araa}{Annual Rev. Astron. Astrophys. }
% *** Astronomicekij Zhurnal
\newcommand{\azh}{Astron.~Zh. }
% *** Bulletin of the American Astron. Society
\newcommand{\baas}{Bull. Amer. Astron. Soc. }
% *** Bulletin of the Special Astrophysical Observatory % англ. версия до 2007 г.
\newcommand{\bsao}{Bull. Spec. Astrophys. Obs. }
% *** Бюллетень Спец. астрофизич. обсерватории % русск. версия до 2007 г.
\newcommand{\bsaor}{Бюлл. Спец. астрофиз. обсерв. }
% *** Inform. Bul. Var. Stars
\newcommand{\ibvs}{Inform. Bull. Var. Stars }
% *** Journal of Astronomy and Astrophysics
\newcommand{\jaa}{J.~Astron. Astrophys. }
% *** Monthly Notices of the Roy. Astron. Society
\newcommand{\mnras}{Monthly Notices Royal Astron. Soc. }
% *** Publ. of the Astron. Society of Australia
\newcommand{\pasa}{Publ. Astron. Soc. Australia }
% *** Publ. Astronom. Soc. Japan
\newcommand{\pasj}{Publ. Astron. Soc. Japan }
% *** Publ. of the Astron. Society of the Pacific
\newcommand{\pasp}{Publ. Astron. Soc. Pacific }
% *** Astronomy Reports (АЖ)
\newcommand{\arep}{Astronomy Reports }
% *** Astronomy Letters (ПАЖ)
\newcommand{\alet}{Astronomy Letters }
% *** Astronomische Nachrichten
\newcommand{\an}{Astronomische Nachrichten }
% *** Pis'ma v Astronomicekij Zhurnal
\newcommand{\pazh}{Pis'ma Astron. Zh. }
% *** Письма в АЖ
\newcommand{\pazhr}{Письма в АЖ }
% *** Астрон. ж.
\newcommand{\azhr}{Астрон.~ж. }
% *** Soviet Astronomy
\newcommand{\sovast}{Sov. Astron. }
% *** Scientific American
\newcommand{\sca}{Scientific American }
% *** Sky and Telescope
\newcommand{\skytel}{Sky Telesc. }
% *** Space Science Reviews
\newcommand{\spsrev}{Space Sci.~Rev. }
% Revista Mexicana de Astronomia y Astrofisica
%\newcommand{\rmxaa}{Revista Mexicana de Astronom\'{\i}a y Astrof\'{\i}sica}
\newcommand{\rmxaa}{Revista Mexicana Astronom. Astrof\'{\i}s. }
%\newcommand{\nat}{Nature }
% *** Physical Review D
\newcommand{\prd}{Phys. Rev.~D }
\newcommand{\memsai}{Memorie della Societ\`a Astronomica Italiana }
% *** Nature
\newcommand{\nat}{Nature }
\newcommand{\aatrans}{Astronomical and Astrophysical Transactions }
\newcommand{\qjras}{Quarterly Journal of the Royal Astronomical Society }
\newcommand{\actaa}{Acta Astronomica }
% *** SPIE Conference Proceedings
\newcommand{\procspie}{SPIE Conf. Proc. }
\newcommand{\na}{New Astronomy }
\newcommand{\apjl}{Astrophys.~J. }
\newcommand{\aapr}{Astron. and Astrophys.}
%
\newcommand{\bain}{Bull. Astron. Inst. Netherlands }
\newcommand{\memras}{Memoirs of the Royal Astronomical Society }
\newcommand{\jqsrt}{Journal of Quantitative Spectroscopy and Radiative Transfer }
%
\newcommand{\jcap}{Journal of Cosmology and Astroparticle Physics }
\newcommand{\physrep}{Physics Reports }

